Towards Automatic Image Editing: Learning to See another You

Learning the distribution of images in order to generate new samples is a challenging task due to the high dimensionality of the data and the highly non-linear relations that are involved. Nevertheless, some promising results have been reported in the literature recently,building on deep network architectures. In this work, we zoom in on a specific type of image generation: given an image and knowing the category of objects it belongs to (e.g. faces), our goal is to generate a similar and plausible image, but with some altered attributes. This is particularly challenging, as the model needs to learn to disentangle the effect of each attribute and to apply a desired attribute change to a given input image, while keeping the other attributes and overall object appearance intact. To this end, we learn a convolutional network, where the desired attribute information is encoded then merged with the encoded image at feature map level. We show promising results, both qualitatively as well as quantitatively, in the context of a retrieval experiment, on two face datasets (MultiPie and CAS-PEAL-R1).

==> training.tex <==

We train the two networks successively.
The input of the first network are the source image of size $32\times32$ and a one-hot vector.
Each image is preprocessed by subtracting the mean and dividing by the standard deviation.
Then we feed the output of the first network and source image as input to the second network.
For both networks, we use Mean Squared Error (MSE) as the loss function,
% loss fucntion equation
\begin{eqnarray}
 & L_1(W_1) = || F_1(X, C_X, W_1) - Y ||_2^2, 
 \\
 & L_2(W_2) = || F_2(X, \hat{Y_1}, W_2) - Y ||_2^2,
\end{eqnarray}

The training parameters are fixed for both networks.
The training is carried out using mini-batch gradient descent with backpropagation~\cite{LeCun-89}
and the batch size is set to 32.
We use the fixed momentum of 0.95 and learning rate of 1e-5.
All the weights are initialized with the method proposed in~\cite{He-iccv15}.



